Neural ODEs with stochastic vector field mixtures

It was recently shown that neural ordinary differential equation models cannot solve fundamental and seemingly straightforward tasks even with high-capacity vector field representations. This paper introduces two other fundamental tasks to the set that baseline methods cannot solve, and proposes mixtures of stochastic vector fields as a model class that is capable of solving these essential problems. Dynamic vector field selection is of critical importance for our model, and our approach is to propagate component uncertainty over the integration interval with a technique based on forward filtering. We also formalise several loss functions that encourage desirable properties on the trajectory paths, and of particular interest are those that directly encourage fewer expected function evaluations. Experimentally, we demonstrate that our model class is capable of capturing the natural dynamics of human behaviour; a notoriously volatile application area. Baseline approaches cannot adequately model this problem.

==> boilerplate.tex <==
\begin{figure}
\centering     %%% not \center
\subfigure[Figure A]{\label{fig:a}\includegraphics[width=60mm]{example-image-a}}
\subfigure[Figure B]{\label{fig:b}\includegraphics[width=60mm]{example-image-b}}
\caption{my caption}
\end{figure}





==> sections/04_related_work.tex <==
\section{Related work}
\label{section:related}



==> sections/99_outline.tex <==
\section*{Outline and main contributins}

\begin{itemize}
    \item Motivate requirement for mixture of VFs -- easy to motivate since it's easy fo find examples which normal ODEs and even AugODEs cannot solve (splitting). Although this breaks the homomorphism that I do agree is definitely important, mixtures of ODEs are still homomorphisms in expectation, and maybe this is enough... (need to prove this, but I think that since expectations are linear operators this should be easy enough)
    \item Motivate requirement uncertainty on the VFs -- depending on how it is set up one can see the uncertainty as corresponding to velocity (ie are you walking faster/slower than expected) or directional undertain (particularly if slight pertebations left and right are not meaningful; important that the left/right uncertainty not fundamentally change the vector field). In my experience I think models trained with uncertainty and tested without seem to be more robust to noise. I * v or sqrt(v) x sqrt(v)' 
    \item advection - moving based on the flow of fluid, ie the transport of a particle based on the field 
    \item Simpler vector fields since the thing can just learn straight lines instead of curves more often than not
    \item is \url{http://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.384.8799&rep=rep1&type=pdf} a bad case in fig 2? the variance is too big
    \item Expressing the variety of models with a Zoubin-like cube: three axes investigated here: augmentation, uncertain vector fields, mixture of vector fields. Augmentation is nice, but can't solve the behavioural modelling problem, and nor can uncertainty. You need mixtures to capture the dynamics of behav models. Uncertainty can help in these situations, however. Augmentation, Uncertainty and Mixtures solve Crossing, Lengthening and Splitting problems. 
    \item Periodic time so that pre- and post-midnight have similar vector fields -- Current ODEs have feature vectors concatenated as such: x -> [x] + [t], and if we are in a setting where t spans a whole day (i.e. 0-24 hours) I think that concatenating the following should force periodic repetition on the representations: x -> [x] + [cos(t), sin(t)] (with appropriate scaling on t to the 0-24 hour scale)
    \item t-sensitivity -- This needs to be investigated a little more than I have yet. It seems that you can get pretty good models with using low values of T, and I have found that using lower values converges quicker and more reliably. I'm not sure how to quantify this so much, however. 
    \item Losses 
    \begin{itemize}
        \item Penalise the length of the flow: it may make sense to prefer minimal transformations of the input data, so that the `broad' statistics of the data are preserved. One can penalise the distance travelled in a couple of ways: 1) penalise the norm of the difference between the original and final transformed point; or 2) penalise the full path length. These points are related with item (1) corresponding to an `as the crow flies' estimation of the full path length and (2) being the full path as the ODE sees it. The latter one is hard enoguh to compute due to how the ODE solver solves the problem
        \item With augmented ODEs, one may want to encourage the model to learn paths with most movement in the augmented dimension. This way one still preserves the broad topology of the original data even in transformation. 
        \item Penalise entropy of component probailities -- encourages a `pick and stick' scenario only changing when the model deems it to be absolutely necessary
        \item Clustering transformed examples of same label -- encourage the trasformed data to cluster
        \item Mixture density loss -- splitting belief over all paths
    \end{itemize}
    \item Is there a relationship between the mixture network and particle filters/reinforcement learning? I can imagine that you may wish to utilise one of these methods in \textit{solving} the problem. Although when forecasting one may choose only a handful of samples, the model has surely been trained with sufficient variety with all samples taken during the learning process. I don't think keeping track of exponentially many paths is then necessary in testing if you learn for enough iterations. 
    \item Component membership 
    \begin{itemize}
        \item Pick once and stick: this is the easiest way of looking at the problem. It says that the main intent of your movement is fully defined at the starting time. In most scenarios I think this is fine. A possible weakness is for people with cog issues that mean they wander, shadow, forget or change their intent. This could lead to more chaotic VFs (or maybe this cannot be modelled?). Need to clarify whether it is the distribution or the sample from the distribution that follows this pick and stick idea. 
        \item Dynamic membership: several options here: 1) use the CRF-like forward filtering approach (this is myopic since the dynamics are more or less well defined by the past); 2) use an exponentially weighted moving average of membership probabilities (this has a nice feature of being a method that is used in forecasting). Democratises the process through the total path
        \item Using gumbel softmax for sampling and preserving gradients through the samples
    \end{itemize}
    \item We are mostly avoiding recurrency in this work -- why? Are there computational advantages? Perhaps we can make the point that in the CRF-like membership dynamics is like an RNN through time. Thinking of the left-or-right dataset, the `pick, sample and stick' idea may make more sense over the `pick and stick and sample'
    \item Context
    \begin{itemize}
        \item Between-resident interactions/relationship -- It should be possible to parameterise these models to capture the degree to how much one resident's location affects the other: are these independent or is there dependence? It may be possible to use something like Granger causality to quantify this (but on forecasts?) 
        \item Can we demonstrate that membership is contextualised by time of day? Can a k-NODE learn that paths up stairs are more likely from the same starting point? 
        \item Model my future based on the forecast of other objects. 
    \end{itemize}
    \item Experiments
    \begin{itemize}
        \item Simple splitting 
        \item Left or right turn
        \item XOR problem (illustrating how component membership is learnt 
        \item Synthetic smart home data 
        \item Real smart home data? (maybe can use MK's?)
        \item Taxi data -- don't know this data enough to really test it... 
        \item Effect of $T$ choice
        \item Learning endpoint uncertainty: learning to move point x to y, and there are several instances of x at the same point in space and each maps to slightly different positions, the mapping will move x to the mean of y, but it is unaware of the variance in its prediction. 
    \end{itemize}
    \item Evaluation
    \begin{itemize}
        \item Number of function evaluations
        \item Complexity of the evaluation -- mixtures don't necessarily require any additional computation
        \item Solving the problem in-space without augmentation 
    \end{itemize}
    \item Forecasting: continuous time optimisation via interpolation of trajectories at time t on ODE solver
    \item what about dropout?
    \item predicting the average without uncertainty is fine, but if you have nonlinear trajectories (eg walking around a corner) predicting the mean may result in predicting outside allowable domain. 
    \item Interpolating in the forecasting case (not in clf/reg)
    \item contributions are on the vector field representations as opposed to augmentation of feature space and NODE solvers. 
    \item Interpolation of points to concatenate losses throughout
    \item Does a SVF with large variance give non-zero probability to all paths?
    \item discussion of time complexity
\end{itemize}
